ChartWalker: Benchmarking the Cross-Chart RAG Task with Hierarchical Knowledge Graphs

Cross-Chart Retrieval-Augmented Generation (RAG) is critical for complex multi-modal analytical tasks in scientific, business, and political domains. However, existing benchmarks either focus on tables, which are well-structured and textualized, or generate cross-chart questions by simply extracting key points, which often induces lexical overlap between queries and evidence and yields logically inconsistent reasoning chains. To address this, we introduce ChartWalker, a novel framework for constructing challenging cross-chart RAG tasks. ChartWalker features a hierarchical knowledge graph construction method tailored to charts, which organizes entities and relations by granularity to preserve analytical structure. We then propose a structure-aware sampling algorithm that synthesizes semantically coherent, multi-hop reasoning paths, enabling explicit control over query difficulty and granularity for QA generation. Built with this framework, we release ChartWalker-Bench, a comprehensive benchmark spanning diverse domains and cross-chart query types. Extensive evaluations across major RAG paradigms reveal significant performance gaps, underscoring the benchmark's difficulty and utility. Furthermore, we provide ChartWalker-Agent, an agentic baseline to facilitate analysis and inspire future system design.

==> cpts/2_pre.tex <==
\section{Preliminary}
% 背景
% 形式化定义

\paragraph{Cross-Chart RAG Task.}
Given a corpus of charts $\mathcal{T}$ and a natural language query $q$ that cannot be directly answered by a pre-trained VLM, we consider a standard retrieval-augmented generation (RAG) pipeline $\mathcal{M}$ operating in two stages.
First, $\mathcal{M}$ retrieves a subset of relevant tables from the corpus.
Second, $\mathcal{M}$ generates an output to support downstream reasoning and answer generation.

Formally, the RAG pipeline is defined as: $\mathcal{T}'=\mathrm{Retrieve}_{\mathcal{M}}(\mathcal{T}, q), Y=\mathrm{Generate}_{\mathcal{M}}(\mathcal{T}', q),$,where $\mathrm{Retrieve}_{\mathcal{M}}(\cdot)$ selects the top-$k$ most relevant tables,
$\mathcal{T}' \subset \mathcal{T}$ denotes the retrieved subset, and
$\mathrm{Generate}_{\mathcal{M}}(\cdot)$ produces an output $Y$ conditioned on both $\mathcal{T}'$ and $q$.


==> cpts/3_method.tex <==
\section{Methodology}
% 方法和挑战对应
% 层次化建图
% 游走
% 分析工具是怎么设计的
\subsection{Hierarchical Chart Graph}

Let $\mathcal{C}$ be the set of charts.
Each chart $c \in \mathcal{C}$ is associated with an image $I_c$ and optional surrounding context $T_c$
(e.g., caption, nearby paragraphs).
We aim to build a global chart knowledge graph (KG) that supports scalable retrieval and cross-chart reasoning.

\paragraph{VLM-based entity extraction.}
Given $(I_c, T_c)$, a VLM extraction module produces a set of entity candidates:
\begin{equation}
    \mathcal{V}_c^{\mathrm{raw}} = f_{\theta}(I_c, T_c),
\end{equation}
where $f_{\theta}$ is prompted to return structured chart elements, including
% (i) global descriptors (title/caption/topic),
% (ii) encoding descriptors (axes, units, legend/series),
% and (iii) fine-grained content (ticks, value annotations, key data points when available). 
Each extracted entity is labeled with a level $\ell(v)$ to measure its granularity with respect to its source info. Lower indices indicate higher retrievability (e.g., title-level concepts may be placed at level $0$).
We then obtain a level-partitioned entity set:
\begin{equation}
    \mathcal{V}_c^{(l)} = \{\, v \in \mathcal{V}_c^{\mathrm{raw}} : \ell(v)=l \,\}, \quad
    \mathcal{V}_c = \bigcup_{l=0}^{L} \mathcal{V}_c^{(l)}.
\end{equation}
Since levels are retrieval-oriented rather than semantic, the \emph{same surface entity may appear in multiple levels},
and we \emph{do not perform cross-level merging}.

\paragraph{Chart subgraph construction.}
For each chart $c$, we construct a chart subgraph
\begin{equation}
    \mathcal{G}_c = (\mathcal{V}_c, \mathcal{E}_c, \mathcal{L}), \qquad \mathcal{L}=\{0,1,\dots,L\},
\end{equation}
where $\mathcal{E}_c$ contains typed edges encoding chart structure and level-aware organization.
We instantiate edges from a fixed relation vocabulary $\mathcal{R}$ and store them as triples $(u,r,v)$.
Concretely, $\mathcal{E}_c$ includes:
\begin{itemize}[leftmargin=*,topsep=0pt,itemsep=1pt]
    \item \textbf{Intra-level relation}: linking title/caption to axes, axes to units/ticks, legends to series, and series to key values when available.
    \item \textbf{Inter-level relation}: connecting a lower-level entity to its higher-level anchor in the same chart
    (e.g., tick $\rightarrow$ axis label $\rightarrow$ chart topic), enabling coarse-to-fine traversal during retrieval.
\end{itemize}

\paragraph{Global KG integration (layer-wise union).}
Let the global KG be $\mathcal{G}=(\mathcal{V},\mathcal{E},\mathcal{L})$ with
$\mathcal{V}=\bigcup_{l}\mathcal{V}^{(l)}$.
We construct $\mathcal{G}$ incrementally by merging chart subgraphs:
\begin{equation}
    \mathcal{G} \leftarrow \mathcal{G} \cup \mathcal{G}_c,
\end{equation}
implemented as level-wise accumulation:
\begin{equation}
    \mathcal{V}^{(l)} \leftarrow \mathcal{V}^{(l)} \cup \mathcal{V}_c^{(l)}, \qquad
    \mathcal{E} \leftarrow \mathcal{E} \cup \mathcal{E}_c.
\end{equation}
This design supports dynamic corpora: new charts can be added by local extraction and local subgraph insertion, without requiring global reconstruction.

\paragraph{Level-wise entity resolution.}
After ingesting a batch $\mathcal{C}_b \subset \mathcal{C}$, we perform \emph{level-wise} consolidation to control noise and redundancy.
For each level $l$, we define a resolution function restricted to that level:
\begin{equation}
    \phi_l(u,v) : \mathcal{V}^{(l)} \times \mathcal{V}^{(l)} \rightarrow \{0,1\},
\end{equation}
where $\phi_l(u,v)=1$ indicates $u$ and $v$ refer to the same real-world entity \emph{within level $l$}.
In practice, $\phi_l$ can combine normalized string matching and embedding similarity under type/unit constraints,
and we cluster entities in $\mathcal{V}^{(l)}$ using union-find to obtain canonical nodes.
We emphasize that \textbf{no cross-level resolution is performed}: even if two entities share the same surface form, they remain distinct if they belong to different levels.

 
\subsection{Data Generation}
\subsubsection{Graph Sampling}

To generate high-quality multi-chart QA pairs, we design a constrained random walk sampler that explores the hierarchical KG $\mathcal{G}$ to discover reasoning paths connecting entities across different charts. Our sampling strategy combines source-weighted PageRank for node importance estimation with multi-branch constrained walks that respect semantic coherence and evidence diversity.

\paragraph{Source-weighted PageRank via Monte Carlo RWR.}
We first compute node importance scores using a Monte Carlo Random Walk with Restart (RWR) procedure that accounts for source rarity and edge type preferences. For each entity $v \in \mathcal{V}$, we define a transition weight $w(v, u)$ for edge $(v, u) \in \mathcal{E}$ as:
\begin{equation}
w(v, u) = w_{\text{rel}}(r) \cdot w_{\text{level}}(v, u, t) \cdot w_{\text{rarity}}(c) \cdot w_{\text{novelty}}(c, S),
\end{equation}
where $r$ is the relation type, $t \in \{\text{horizontal}, \text{vertical\_down}, \text{vertical\_up}\}$ is the move type, $c$ is the source chunk ID associated with edge $(v, u)$, and $S$ is the set of sources already visited in the current walk. Specifically:
\begin{itemize}[leftmargin=*,topsep=0pt,itemsep=1pt]
    \item $w_{\text{rel}}(r)$: fixed relation type weight (default: 1.0 for horizontal, 1.5 for vertical\_down, 0.5 for vertical\_up).
    \item $w_{\text{level}}(v, u, t)$: level transition preference, encouraging downward traversal when $t = \text{vertical\_down}$.
    \item $w_{\text{rarity}}(c) = 1 / \sqrt{\max(1, f(c))}$: inverse square root of source frequency $f(c)$, promoting rare sources.
    \item $w_{\text{novelty}}(c, S) = 1 + \lambda$ if $c \notin S$, else $1$: novelty bonus $\lambda$ for unvisited sources.
\end{itemize}

We perform $N_{\text{walks}}$ Monte Carlo walks of length $L_{\text{walk}}$ from seed entities sampled from top-$k$ degree-ranked nodes. Each walk restarts with probability $p_{\text{restart}}$ to balance exploration and exploitation. The PageRank score $\pi(v)$ for entity $v$ is the normalized visit frequency across all walks:
\begin{equation}
\pi(v) = \frac{\text{count}(v)}{\sum_{u \in \mathcal{V}} \text{count}(u)},
\end{equation}
where $\text{count}(v)$ is the number of times $v$ is visited during the Monte Carlo simulation.

\paragraph{Multi-branch path sampling.}
Given a sampled center entity $v_0$ (anchor), we generate $B$ branches $\{\mathcal{P}_1, \ldots, \mathcal{P}_B\}$, where each branch $\mathcal{P}_i$ is a path starting from $v_0$ and ending at an endpoint entity $v_i^{\text{end}}$. Each branch is generated via a constrained random walk that:
\begin{enumerate}[leftmargin=*,topsep=0pt,itemsep=2pt]
    \item \textbf{Starts from center}: All branches originate from the same center entity $v_0$ to ensure coherent reasoning.
    \item \textbf{Applies source-level pruning}: No source chunk $c$ appears twice within the same branch, i.e., for branch $\mathcal{P}_i = [e_1, \ldots, e_n]$ with edges $e_j$ having sources $c_j$, we require $c_j \neq c_k$ for $j \neq k$.
    \item \textbf{Avoids immediate backtracking}: If the walk moves from $v$ to $u$ via source $c$, it cannot immediately return from $u$ to $v$ via the same source $c$.
    \item \textbf{Enforces semantic coherence}: When entity embeddings are available, we compute a branch vector $\mathbf{b}_i$ (either the endpoint embedding or the average of all entity embeddings in the branch) and require cosine similarity $\text{sim}(\mathbf{b}_1, \mathbf{b}_i) \geq \tau$ for $i > 1$, where $\tau$ is a semantic threshold.
\end{enumerate}

For each step in branch $\mathcal{P}_i$, we select the next entity $u$ from neighbors of current entity $v$ using weighted sampling, where the weight combines:
\begin{equation}
w_{\text{sample}}(v, u) = (1 + \beta \cdot \pi(u)) \cdot w_{\text{level}}(v, u, t) \cdot w_{\text{novelty}}(c, S_i) \cdot w_{\text{sem}}(v_0, u),
\end{equation}
where $\beta$ controls PageRank attraction, $S_i$ is the set of sources used in branch $\mathcal{P}_i$ so far, and $w_{\text{sem}}(v_0, u) = 1 + \gamma \cdot \text{sim}(\mathbf{e}_{v_0}, \mathbf{e}_u)$ if semantic embeddings $\mathbf{e}_{v_0}, \mathbf{e}_u$ are available (with $\gamma \geq 0$ controlling semantic influence). The level weight $w_{\text{level}}$ encourages downward traversal (prefer\_down=True) to reach more specific entities.

\paragraph{Path validation and filtering.}
A sampled path configuration $\mathcal{P} = \{v_0, \{\mathcal{P}_1, \ldots, \mathcal{P}_B\}\}$ is accepted only if it satisfies:
\begin{itemize}[leftmargin=*,topsep=0pt,itemsep=1pt]
    \item \textbf{Source diversity}: The union of all sources across branches $\bigcup_{i=1}^B S_i$ contains at least $M_{\text{min}}$ distinct sources.
    \item \textbf{Chart requirement}: At least $M_{\text{chart}}$ sources are chart chunks (i.e., $c$ starts with ``chart\_'').
    \item \textbf{Branch uniqueness}: No branch is a prefix of another (prevents redundant paths).
    \item \textbf{Endpoint diversity}: All branch endpoints are distinct entities.
\end{itemize}

If validation fails, we retry sampling up to $R_{\text{retry}}$ times with a new center entity. The final path structure $\mathcal{P}$ provides the reasoning chain connecting entities across multiple charts, which serves as input to the QA generation module.

\subsubsection{QA Generation from Sampled Paths}

Given a sampled path configuration $\mathcal{P} = \{v_0, \{\mathcal{P}_1, \ldots, \mathcal{P}_B\}\}$, we generate a multi-chart QA pair through a one-pass VLM-based generation procedure. The process involves evidence selection, prompt construction, and type-specific question formulation.

\paragraph{Evidence selection and formatting.}
We first extract evidence sources from the sampled paths. Let $S = \bigcup_{i=1}^B S_i$ be the union of all source chunks across branches. We prioritize chart sources over text sources, selecting up to $M_{\text{max}}$ evidence items:
\begin{equation}
\mathcal{E}_{\text{selected}} = [c_1, \ldots, c_{n_c}, t_1, \ldots, t_{n_t}], \quad n_c + n_t \leq M_{\text{max}},
\end{equation}
where $c_i$ are chart chunk IDs and $t_i$ are text chunk IDs, with charts appearing first. For each chart $c_i$, we retrieve its image $I_{c_i}$ and create a chart index mapping $\text{idx}: c_i \mapsto i$ that allows the model to reference charts by image position. Text chunks are formatted as snippets with chunk ID annotations.

\paragraph{Query type classification and prompt selection.}
Our system supports four query types distinguished by their reasoning requirements:
\begin{itemize}[leftmargin=*,topsep=0pt,itemsep=1pt]
    \item \textbf{FactCheck}: Verify a factual claim using evidence from multiple sources. The question asks whether a statement is true or false based on the provided evidence.
    \item \textbf{Manipulation}: Require numerical calculations on extracted data, such as percentage-point differences, ratios, aggregations (sums of categories), rankings, or threshold comparisons. These questions demand computational reasoning beyond simple lookup.
    \item \textbf{Trend}: Describe temporal changes or patterns visible across charts, requiring identification of increases, decreases, or stable trends over time.
    \item \textbf{Analysis}: Multi-hop and multi-source analytical reasoning that connects concepts across different domains, time periods, or population groups, exploring logical relationships and implications.
\end{itemize}

We employ three specialized prompt variants, each optimized for generating different question categories:
\begin{enumerate}[leftmargin=*,topsep=0pt,itemsep=2pt]
    \item \textbf{QA\_OnePass\_easy}: Designed for generating \textbf{FactCheck} and \textbf{Manipulation} questions. This prompt requires combining evidence from at least \textbf{two} different sources and focuses on straightforward verification or computational tasks without complex multi-hop reasoning. It excludes the Analysis query type to maintain simplicity.
    \item \textbf{QA\_OnePass}: Tailored for generating more complex \textbf{Trend} and \textbf{Analysis} questions that require deeper analytical reasoning. While it supports all four query types, it emphasizes analytical depth, connecting concepts across domains and exploring logical relationships. It requires at least \textbf{two} sources and avoids direct chart title references.
    \item \textbf{QA\_OnePass\_long}: Specialized for generating long-hop reasoning questions with narrative chain structures. It mandates at least \textbf{three} different sources and enforces a narrative chain where each sentence connects to the previous one (e.g., ``This...'', ``The...'', ``Within this...''), creating a coherent multi-hop narrative rather than using ``Considering X...'' format. This prompt also includes an \emph{Entity-Answer Alignment} constraint: every entity mentioned in the question must be used in the answer with specific data. It supports all four query types but is particularly effective for complex Analysis questions requiring extended reasoning chains.
\end{enumerate}

\paragraph{One-pass generation with VLM.}
Given the selected prompt template $T$ (one of the three variants), we construct the input prompt by formatting:
\begin{itemize}[leftmargin=*,topsep=0pt,itemsep=1pt]
    \item \textbf{reasoning\_paths}: The formatted branch structure showing level transitions (e.g., L0→L1→L2) and entity connections.
    \item \textbf{available\_sources}: The list of selected chunk IDs.
    \item \textbf{chart\_index}: The mapping from image index to chunk ID for chart citation.
    \item \textbf{text\_evidence}: Formatted text snippets with chunk ID annotations.
\end{itemize}

The VLM (e.g., Qwen3-VL-235B) processes the prompt along with chart images $\{I_{c_1}, \ldots, I_{c_{n_c}}\}$ and generates a structured JSON output containing:
\begin{equation}
\text{QA} = \{\text{query\_type}, \text{question}, \text{answer}, \text{explanation}, \text{entities\_used}, \text{evidence}, \text{evidence\_charts}, \text{difficulty\_subjective}\},
\end{equation}
where $\text{query\_type} \in \{\text{FactCheck}, \text{Manipulation}, \text{Trend}, \text{Analysis}\}$ (subject to prompt constraints), $\text{question}$ is self-contained and avoids revealing specific numerical values, $\text{answer}$ provides a definitive response with specific data, and $\text{evidence\_charts}$ cites charts using the image index mapping.

\paragraph{Answer verification (optional).}
To ensure quality, we optionally verify each generated answer by prompting the VLM to fact-check the answer against the evidence. If verification fails, we retry generation up to $R_{\text{retry}}$ times with the same path configuration before accepting or discarding the QA pair.

\TN{Decontextualization}

\subsection{Visual Searching Agent}
\TN{To Further XXX} we train a visual search agent with a small set of primitive graph actions. 
The agent learns to adopt different search strategies under different scenarios---e.g., deep multi-hop traversal for relational queries versus breadth-oriented evidence aggregation for entity-centric queries---and to collect sufficient evidence before producing an answer. 

\paragraph{Visual Multi Turn RL}
\paragraph{Action Space}
\paragraph{Reward Design}
